Multilingual and Explainable Text Detoxification with Parallel Corpora

Even with various regulations in place across countries and social media platforms (Government of India, 2021; European Parliament and Council of the European Union, 2022, digital abusive speech remains a significant issue. One potential approach to address this challenge is automatic text detoxification, a text style transfer (TST) approach that transforms toxic language into a more neutral or non-toxic form. To date, the availability of parallel corpora for the text detoxification task (Logachevavet al., 2022; Atwell et al., 2022; Dementievavet al., 2024a) has proven to be crucial for state-of-the-art approaches. With this work, we extend parallel text detoxification corpus to new languages -- German, Chinese, Arabic, Hindi, and Amharic -- testing in the extensive multilingual setup TST baselines. Next, we conduct the first of its kind an automated, explainable analysis of the descriptive features of both toxic and non-toxic sentences, diving deeply into the nuances, similarities, and differences of toxicity and detoxification across 9 languages. Finally, based on the obtained insights, we experiment with a novel text detoxification method inspired by the Chain-of-Thoughts reasoning approach, enhancing the prompting process through clustering on relevant descriptive attributes.

==> paradetox_per_lang/english.tex <==
\subsection{English}
\label{sec:english}

For English, we reused the data from English ParaDetox dataset~\cite{logacheva-etal-2022-paradetox} and additionally manually marked up approximately 400 pairs to form a validation dataset of 1000 examples.   

\subsubsection{Input Data Preparation}

For EnParaDetox, the original toxic texts were taken from Jigsaw toxicity identification challenge train dataset~\cite{jigsaw}. We have 
considered only texts labeled as \texttt{toxic} and \texttt{severe toxic}.  

\subsubsection{Annotation Process} 

The training and validation sets of EnParaDetox were acquired through crowdsourcing via Toloka\footnote{\href{https://toloka.ai}{https://toloka.ai}} platform with fluent English speakers. Additionally, we employed annotators who are fluent in English and hold a Masters degree in Computer Science to compile additional samples to the test set.

% \paragraph{Annotation Task(s)} We adapt ParaDetox \cite{DBLP:conf/acl/LogachevaDUMDKS22} collection pipeline as it was designed to automate the data collection as well as verification with crowdsourcing. The pipeline consists of three tasks: 
% \begin{description}
% \item[\textbf{Task 1: Rewrite text in a polite way}] Annotators need to provide the detoxified paraphrase of the text so it becomes non-toxic and the main content is saved or to skip paraphrasing if the text is not possible to rewrite in non-toxic way; 
% \item[\textbf{Task 2: Do these sentences mean the same?}] Check if the content is indeed the same between the original toxic text and its potential non-toxic paraphrase; 
% \item[\textbf{Task 3: Is this text offensive?}] Verification of the provided paraphrase if it is indeed non-toxic.
% \end{description}

% \paragraph{Annotation Instructions} + all details in Appendix~\ref{sec:app_instructions} for the corresponding language.

% \paragraph{Annotators} General info and demographics about annotators.

% \paragraph{Annotation Process} Annotation Tool + Annotation Interface + quality controls

==> paradetox_per_lang/russian.tex <==
\subsection{Russian}
\label{sec:russian}

The same as for English, there were previously available training and validation data from previous work~\cite{Dementieva2022RUSSE2022FO,dementieva2024multiparadetox}. We reused this data and manually annotated some additional toxic examples taken from various toxicity datasets.

% \subsubsection{Input Data Preparation}

% In addition to 856 text pairs taken from the RUSSE 2022 test part, we have manually detoxified 300 more text pairs. We then manually selected best text pairs to form a resulting parallel detoxification dataset of 1000 sentence pairs.   

\paragraph{Input Toxicity Data} The original toxic samples were taken from two binary toxicity classification Kaggle Toxic Comments datasets~\cite{tox_ru_comments_1,tox_ru_comments_2}. 

% \paragraph{Input Preprocessing} We re-evaluated the toxicity of the samples with the toxicity classifier from~\cite{DBLP:conf/ijcnlp/DementievaMDP23} and manually filtered the texts to be between 5 and 30 works each. 


\subsubsection{Annotation Process}

The training and validation sets of RuParaDetox were acquired through crowdsourcing via Toloka platform with fluent Russian speakers. Additionally, we employed annotators who are native in Russian and hold a Masters degree in Computer Science to compile additional samples to the test set.

% The annotator was a PhD student in Computer Science with Russian language being native. The annotator followed the instructions presented in~\cite{logacheva-etal-2022-paradetox}. 

% \paragraph{Annotation Instructions} + all details in Appendix~\ref{sec:app_instructions} for the corresponding language.

% \paragraph{Annotators} General info and demographics about annotators.

% \paragraph{Annotation Process} Annotation Tool + Annotation Interface + quality controls

==> paradetox_per_lang/spanish.tex <==
\subsection{Spanish}
\label{sec:spanish}

We used the data presented in MultiParaDetox paper~\cite{dementieva2024multiparadetox} providing the main details of data collection:

% \subsubsection{Input Data Preparation}

\paragraph{Input Toxicity Data} For Spanish, we selected samples for annotation from three datasets: hate speech detection ones~\cite{DBLP:journals/sensors/Pereira-Kohatsu19,taule2024newscom} as well as filtered by keywords Spanish Tweets corpus~\cite{perez-etal-2022-robertuito}.

% \paragraph{Input Preprocessing}

\subsubsection{Annotation Process}

% \paragraph{Annotation Instructions} + all details in Appendix~\ref{sec:app_instructions} for the corresponding language.

% \paragraph{Annotators} General info and demographics about annotators.

% \paragraph{Annotation Process} Annotation Tool + Annotation Interface + quality controls

We adapt ParaDetox \cite{DBLP:conf/acl/LogachevaDUMDKS22} collection pipeline and verified the data quality via crowdsourcing. We utilized the Toloka platform for crowdsourcing tasks in Ukrainian. The annotators, who were native Spanish speakers, underwent an examination before starting the tasks.

==> paradetox_per_lang/ukrainian.tex <==
\subsection{Ukrainian}
\label{sec:ukrainian}

We used the data presented in MultiParaDetox paper~\cite{dementieva2024multiparadetox} providing the main details of data collection:

% \subsubsection{Input Data Preparation}

\paragraph{Input Toxicity Data} For the Ukrainian language, there was no existing binary toxicity classification corpus. Therefore, we filtered explicitly toxic samples containing obscene lexicon from the predefined list~\cite{tox_uk_lexicon} within the Ukrainian Tweets Corpus~\cite{bobrovnyk2019automated}.

% \paragraph{Input Preprocessing}

\subsubsection{Annotation Process}

% \paragraph{Annotation Instructions} + all details in Appendix~\ref{sec:app_instructions} for the corresponding language.

% \paragraph{Annotators} General info and demographics about annotators.

% \paragraph{Annotation Process} Annotation Tool + Annotation Interface + quality controls

We adapt ParaDetox \cite{DBLP:conf/acl/LogachevaDUMDKS22} collection pipeline and verified the data quality via crowdsourcing. We utilized the Toloka platform for crowdsourcing tasks in Ukrainian. The annotators, who were native Ukrainian speakers, underwent an examination before starting the tasks.
